TEDDY: Trimming Edges with Degree-based Discrimination strategY

Since the pioneering work on the lottery ticket hypothesis for graph neural networks (GNNs) was proposed in Chen et al. (2021), the study on finding graph lottery tickets (GLT) has become one of the pivotal focus in the GNN community, inspiring researchers to discover sparser GLT while achieving comparable performance to original dense networks. In parallel, the graph structure has gained substantial attention as a crucial factor in GNN training dynamics, also elucidated by several recent studies. Despite this, contemporary studies on GLT, in general, have not fully exploited inherent pathways in the graph structure and identified tickets in an iterative manner, which is time-consuming and inefficient. To address these limitations, we introduce TEDDY, a one-shot edge sparsification framework that leverages structural information by incorporating edge-degree information. Following edge sparsification, we encourage the parameter sparsity during training via simple projected gradient descent on the $\ell_0$ ball. Given the target sparsity levels for both the graph structure and the model parameters, our TEDDY facilitates efficient and rapid realization of GLT within a single training. Remarkably, our experimental results demonstrate that TEDDY significantly surpasses conventional iterative approaches in generalization, even when conducting one-shot sparsification that solely utilizes graph structures, without taking feature information into account.

==> table_graphspar.tex <==
{\renewcommand{\arraystretch}{1.4}
% \begin{table*}[hbt!]
  \begin{table*}[t!]
    \caption{\blue{A sole graph sparsification performance (in percentage) of proposed method, high degree-based pruning, and baselines.}}
    \vskip -10pt
    % {\LARGE
    \centering
    % \resizebox{.95\textwidth}{!}{
    \resizebox{0.95\textwidth}{!}{
    \footnotesize{
    \begin{tabular}{ c | c | c | c | c | c | c }
     \hline\hline
     \textbf{Simulations} & \textbf{Methods} & \textbf{1-th} & \textbf{5-th} & \textbf{10-th} & \textbf{15-th} & \textbf{20-th} \\
     \hline
     % \multirow{3}{*}{Acc.} &
     \multirow{4}{*}{Cora} 
     & {UGS}
     & {71.83 \fontsize{8}{9}\selectfont$\pm$ 2.75}
     & {69.83 \fontsize{8}{9}\selectfont$\pm$ 2.96}
     & {68.27 \fontsize{8}{9}\selectfont$\pm$ 2.18} 
     & {68.53 \fontsize{8}{9}\selectfont$\pm$ 2.15}
     & {67.60 \fontsize{8}{9}\selectfont$\pm$ 2.49} \\

     & {WD-GLT}
     & {76.83 \fontsize{8}{9}\selectfont$\pm$ 0.31}
     & {75.47 \fontsize{8}{9}\selectfont$\pm$ 0.05}
     & {73.80 \fontsize{8}{9}\selectfont$\pm$ 0.93} 
     & {71.43 \fontsize{8}{9}\selectfont$\pm$ 1.47}
     & {70.97 \fontsize{8}{9}\selectfont$\pm$ 1.23} \\

     & \textbf{Ours}
     & {73.24 \fontsize{8}{9}\selectfont$\pm$ 0.36}
     & \textbf{77.60 \fontsize{8}{9}\selectfont$\pm$ 0.24}
     & \textbf{76.52 \fontsize{8}{9}\selectfont$\pm$ 0.27} 
     & \textbf{76.48 \fontsize{8}{9}\selectfont$\pm$ 0.28}
     & \textbf{75.78 \fontsize{8}{9}\selectfont$\pm$ 0.19} \\

     & {High degree-based}
     & \textbf{77.52 \fontsize{8}{9}\selectfont$\pm$ 0.59}
     & {77.54 \fontsize{8}{9}\selectfont$\pm$ 1.86}
     & {75.10 \fontsize{8}{9}\selectfont$\pm$ 1.46} 
     & {73.76 \fontsize{8}{9}\selectfont$\pm$ 0.81}
     & {70.90 \fontsize{8}{9}\selectfont$\pm$ 1.01} \\
     \hline
     \multirow{4}{*}{Citeseer} 
     & {UGS}
     & {64.80 \fontsize{8}{9}\selectfont$\pm$ 2.02}
     & {65.57 \fontsize{8}{9}\selectfont$\pm$ 3.35}
     & {65.37 \fontsize{8}{9}\selectfont$\pm$ 2.08} 
     & {64.47 \fontsize{8}{9}\selectfont$\pm$ 1.86}
     & {63.50 \fontsize{8}{9}\selectfont$\pm$ 1.84} \\

     & {WD-GLT}
     & {63.93 \fontsize{8}{9}\selectfont$\pm$ 2.90}
     & {64.63 \fontsize{8}{9}\selectfont$\pm$ 2.38}
     & {62.93 \fontsize{8}{9}\selectfont$\pm$ 2.90} 
     & {63.60 \fontsize{8}{9}\selectfont$\pm$ 1.92}
     & {62.57 \fontsize{8}{9}\selectfont$\pm$ 1.50} \\

     & \textbf{Ours}
     & \textbf{69.64 \fontsize{8}{9}\selectfont$\pm$ 0.48}
     & {68.96 \fontsize{8}{9}\selectfont$\pm$ 0.15}
     & {68.78 \fontsize{8}{9}\selectfont$\pm$ 0.20} 
     & \textbf{68.75 \fontsize{8}{9}\selectfont$\pm$ 0.19}
     & \textbf{68.58 \fontsize{8}{9}\selectfont$\pm$ 0.17} \\

     & {High degree-based}
     & {67.92 \fontsize{8}{9}\selectfont$\pm$ 1.14}
     & \textbf{68.98 \fontsize{8}{9}\selectfont$\pm$ 0.62}
     & \textbf{68.80 \fontsize{8}{9}\selectfont$\pm$ 0.58} 
     & {67.08 \fontsize{8}{9}\selectfont$\pm$ 0.17}
     & {65.52 \fontsize{8}{9}\selectfont$\pm$ 1.03} \\
     \hline

     \multirow{4}{*}{Pubmed} 
     & {UGS}
     & {72.57 \fontsize{8}{9}\selectfont$\pm$ 1.93}
     & {74.70 \fontsize{8}{9}\selectfont$\pm$ 2.94}
     & {74.37 \fontsize{8}{9}\selectfont$\pm$ 2.25} 
     & {73.27 \fontsize{8}{9}\selectfont$\pm$ 2.01}
     & {72.43 \fontsize{8}{9}\selectfont$\pm$ 2.03} \\

     & {WD-GLT}
     & {76.43 \fontsize{8}{9}\selectfont$\pm$ 1.22}
     & {76.33 \fontsize{8}{9}\selectfont$\pm$ 2.19}
     & {77.50 \fontsize{8}{9}\selectfont$\pm$ 0.99} 
     & {75.87 \fontsize{8}{9}\selectfont$\pm$ 0.60}
     & {75.47 \fontsize{8}{9}\selectfont$\pm$ 0.66} \\

     & \textbf{Ours}
     & \textbf{78.66 \fontsize{8}{9}\selectfont$\pm$ 0.17}
     & \textbf{78.44 \fontsize{8}{9}\selectfont$\pm$ 0.39}
     & \textbf{78.18 \fontsize{8}{9}\selectfont$\pm$ 0.35} 
     & \textbf{77.54 \fontsize{8}{9}\selectfont$\pm$ 0.34}
     & \textbf{77.14 \fontsize{8}{9}\selectfont$\pm$ 0.33} \\

     & {High degree-based}
     & {78.12 \fontsize{8}{9}\selectfont$\pm$ 0.43}
     & {77.36 \fontsize{8}{9}\selectfont$\pm$ 0.39}
     & {76.78 \fontsize{8}{9}\selectfont$\pm$ 1.25} 
     & {74.82 \fontsize{8}{9}\selectfont$\pm$ 0.58}
     & {73.00 \fontsize{8}{9}\selectfont$\pm$ 0.51} \\
     \hline\hline
     \end{tabular}
     \label{tab:overall_graphspar}
     }
     }
     \vskip -10pt
    \end{table*}
}
